Neural Subgraph Matching

Subgraph matching is the problem of determining the presence and location(s) of a given query graph in a large target graph. Despite being an NP-complete problem, the subgraph matching problem is crucial in domains ranging from network science and database systems to biochemistry and cognitive science. However, existing techniques based on combinatorial matching and integer programming cannot handle matching problems with both large target and query graphs. Here we propose NeuroMatch, an accurate, efficient, and robust neural approach to subgraph matching. NeuroMatch decomposes query and target graphs into small subgraphs and embeds them using graph neural networks. Trained to capture geometric constraints corresponding to subgraph relations, NeuroMatch then efficiently performs subgraph matching directly in the embedding space. Experiments demonstrate NeuroMatch is 100x faster than existing combinatorial approaches and 18% more accurate than existing approximate subgraph matching methods.

==> ack.tex <==
\section{Acknowledgement}
The authors acknowledge Andrew Wang (anwang@cs.stanford.edu) for helping with code organization and integration with the PyTorch Geometric and DeepSNAP libraries.
We gratefully acknowledge the support of
DARPA under Nos. FA865018C7880 (ASED), N660011924033 (MCS);
ARO under Nos. W911NF-16-1-0342 (MURI), W911NF-16-1-0171 (DURIP);
NSF under Nos. OAC-1835598 (CINES), OAC-1934578 (HDR), CCF-1918940 (Expeditions), IIS-2030477 (RAPID);
Stanford Data Science Initiative, 
Wu Tsai Neurosciences Institute,
Chan Zuckerberg Biohub,
Amazon, Boeing, Chase, Docomo, Hitachi, Huawei, JD.com, NVIDIA, Dell. 
J. L. is a Chan Zuckerberg Biohub investigator.



==> broader_impact.tex <==
\newpage
\section{Broader Impact}

Subgraph matching is a problem of fundamental theoretical importance in computer science, and finds applications in a broad range of disciplines where graph processing arises. In social science, social networks are commonly modeled as large graphs, and subgraph analysis has played an important role in the analysis of network effects \cite{leskovec2006patterns}. Information retreival systems use subgraph structures in knowledge graphs for semantic summarization, analogy reasoning, and relationship prediction \cite{gentner1983structure, song2018mining}. In chemistry, subgraph matching is a robust and accurate method for determining similarity between chemical compounds, a necessary precursor for recent methods in chemical retrosynthesis as well as analysis of complex chemical reactions in systems biology \cite{raymond2002heuristics, dai2019retrosynthesis}. Elsewhere in biology, subgraph matching is of central importance in the analysis of protein-protein interaction networks, where identifying and predicting functional motifs is a primary tool for understanding biological mechanisms such as those underlying disease, aging, and medicine \cite{alon2008biomolecular, shen2012mining}. An efficient, accurate model for the subgraph matching problem such as \name could drive research in all of these domains, by providing insights into important substructures of these networks, which have traditionally been limited by either the quality of their approximate algorithms or the runtime of exact algorithms.

While the model itself is widely applicable, its application into these disciplines requires caution. Since queries are typically detemined at inference time, it is easy for human biases (based on observed inference data) to leak into the queries and bias results, confirming hypotheses while missing other important subgraph patterns which do not support the hypothesis. Moreover, a GNN-generated output should be treated with the same scrutiny as any other research result; our model is still imperfect and likely always will be. With the deleterious societal effects of automation bias and algorithmic bias becoming increasingly clear, care must be taken to ensure that results are validated with due diligence.

From a theoretical perspective, our work additionally demonstrates the possibility to learn accurate models for NP-hard problems on graphs. Hence, it could inspire other high-performance GNN-based approaches to similar hard graph problems such as vertex cover, independent set, Hamiltonian paths, \emph{etc.}. These problems are widely used in areas such as operations research, computer systems and architecture. Future work in these related problems has the potential to revolutionize these fields.

